Measurement of Ratios of $\nu_{\mu}$ Charged-Current Cross Sections on C, Fe, and Pb to CH at Neutrino Energies 2-20 GeV

We present measurements of $\nu_{\mu}$ charged-current cross section ratios on carbon, iron, and lead relative to a scintillator (CH) using the fine-grained MINERvA detector exposed to the NuMI neutrino beam at Fermilab. The measurements utilize events of energies $2<E_{\nu}<20~GeV$, with $\left< E_{\nu}\right>=8~GeV$, which have a reconstructed $\mu^{-}$ scattering angle less than $17^\circ$ to extract ratios of inclusive total cross sections as a function of neutrino energy $E_{\nu}$ and flux-integrated differential cross sections with respect to the Bjorken scaling variable $x$. These results provide the first high-statistics direct measurements of nuclear effects in neutrino scattering using different targets in the same neutrino beam. Measured cross section ratios exhibit a relative depletion at low $x$ and enhancement at large $x$. Both become more pronounced as the nucleon number of the target nucleus increases. The data are not reproduced by GENIE, a conventional neutrino-nucleus scattering simulation, or by the alternative models for the nuclear dependence of inelastic scattering that are considered.

==> replacement_table_I.tex <==
\begingroup
\squeezetable
\begin{table}
\begin{tabular}{cccccccc}
\hline \hline
Reconstructed \Xbj & I    & II   & III  & IV   & V    & Mean Generated \Qsq\\
                   & (\%) & (\%) & (\%) & (\%) & (\%) &  (\GeVcsq)\\
\hline
0.0--0.1 & 11.3    &  42.5    &  5.9   &  19.2  & 15.7  &  0.23 \\
0.1--0.3 & 13.6    &  36.4    &  16.7  &  9.1   & 23.0  &  0.70 \\
0.3--0.7 & 32.7    &  32.8    &  11.8  &  1.4   & 21.1  &  1.00 \\
0.7--0.9 & 55.1    &  25.4    &  4.3   &  0.5   & 14.6  &  0.95 \\
0.9--1.1 & 62.7    &  21.6    &  2.8   &  0.5   & 12.3  &  0.90 \\
1.1--1.5 & 69.6    &  18.1    &  1.9   &  0.4   & 9.9   &  0.82 \\
$>1.5$   & 79.1    &  12.8    &  0.6   &  0.3   & 7.1   &  0.86 \\
\hline \hline
\end{tabular}
\caption{
  Average sample composition of selected nuclear target and tracker events in reconstructed \Xbj bins
  based on GENIE simulation of different physics processes, together with the average generated \Qsq.
  Processes are (I) quasielastic, (II) baryon resonance production, (III) deep inelastic scattering at $\Qsq>1$~\GeVcsq and $W>2$~\GeV, (IV) deep inelastic scattering at $\Qsq<1$~\GeVcsq and $W>2$~\GeV, and (V) nonresonant inelastic continuum with $W<2$~\GeV.
} 
\label{tab:sample_comp_Summary_table}
\end{table}
\endgroup

